Adaptive Generation of Phantom Limbs Using Visible Hierarchical Autoencoders

This paper proposed a hierarchical visible autoencoder in the adaptive phantom limbs generation according to the kinetic behavior of functional body-parts, which are measured by heterogeneous kinetic sensors. The proposed visible hierarchical autoencoder consists of interpretable and multi-correlated autoencoder pipelines, which is directly derived from the hierarchical network described in forest data-structure. According to specified kinetic script (e.g., dancing, running, etc.) and users' physical conditions, hierarchical network is extracted from human musculoskeletal network, which is fabricated by multiple body components (e.g., muscle, bone, and joints, etc.) that are bio-mechanically, functionally, or nervously correlated with each other and exhibit mostly non-divergent kinetic behaviors. Multi-layer perceptron (MLP) regressor models, as well as several variations of autoencoder models, are investigated for the sequential generation of missing or dysfunctional limbs. The resulting kinematic behavior of phantom limbs will be constructed using virtual reality and augmented reality (VR/AR), actuators, and potentially controller for a prosthesis (an artificial device that replaces a missing body part). The addressed work aims to develop practical innovative exercise methods that (1) engage individuals at all ages, including those with a chronic health condition(s) and/or disability, in regular physical activities, (2) accelerate the rehabilitation of patients, and (3) release users' phantom limb pain. The physiological and psychological impact of the addressed work will critically be assessed in future work.

==> backup/7.phantomLimb.tex <==
\section{Generation of Phantom Limbs inferred}
\label{subsection:compensationMissingData}
\vspace{2mm}
\subsection{Implementation Mechanism.}
{\em Partial control} is an important feature of VIGOR because it enables those users with disability to operate VIGOR freely. Partial control is implemented by compensating the missing data inferred by disabled input channels: 
in the event that several input channels are disabled,  the VIGOR model is able to construct the void input channels by taking the advantage of correlation among all inputs. 
Compensation can normalize the input data so that VIGOR can achieve higher recognition rate, its psychological and physiological benefits to users are also under our investigation.  


% \begin{wrapfigure}{L}{0.45\textwidth}
%     \centering
%     \includegraphics[width=0.43\textwidth]{figures/fig16-CompensateDisabledChannels.jpg}
% 	\caption{Compensation of disabled input channels via Deep Neural Network (DNN)}
% 	\label{Fig16-CompensateDisabledChannels}
% \end{wrapfigure}
%
\begin{figure}[htp]
 	\centering
	\includegraphics[height=3.5 cm]{figures/fig16-CompensateDisabledChannels.jpg}
	\includegraphics[height=3.5 cm]{figures/fig16b-partialcontrol-demo.png}
	\includegraphics[height=3.5 cm]{figures/fig16G-MLP-phantomLegs.jpg}
	\caption{Compensation of disabled input channels via Deep Neural Network: (a) framework; (b) snapshot about the compensated kinetic status of a wheel-chaired user, who receives ``functional phantom legs'' (in yellow color) through disable-channel compensation;  (c) walking by moving arms (online video \cite{online13-Dakila-Autoencoder-PhantomLeg2018}) % https://www.youtube.com/watch?v=BFW3JVI0dKM )
	}
	\label{Fig16-CompensateDisabledChannels}
\end{figure} 

As illustrated in Figure \ref{Fig16-CompensateDisabledChannels}(a), $x_1$, $x_2$, $x_3$, and $x_4$ constitute the four input channels while the lower-limb-related input $x_4$ is not valid for a seated user. Fortunately, we can formulate $x_4$ according to the correlation between $x_4$ and other enabled inputs -- $x_1$, $x_2$, and $x_3$. The correlation can be discovered using a supervised deep neural network (DNN) regression \cite{Bengio2009,Sperduti1997}, based on which the input $x_4$ can be reconstructed as a function of other known inputs: $x_4' = DNN(x_1,x_2,x_3) $;  the training data comes from the recorded virtual Tai-Chi master's kinematic data. As our preliminary contribution, MLP and autoencoder methods are employed to construct phantom legs according to arm kinetics.

Figure \ref{Fig16-CompensateDisabledChannels}(b) shows a snapshot about the compensated kinetic status of a wheel-chair-bound user, who received ``phantom functional legs'' through compensation of missing data that is related to user's non-functional legs. Besides expediting gesture recognition to be addressed in Section \ref{Section:MeasureRecognitionTimeSeries}, missing data compensation has potential clinical benefit to users. As addressed in \cite{Ortiz-2016-Phantom-Pain}, phantom motor execution facilitated by deep learning and augmented reality can be employed as a treatment for phantom limb pain.

\subsection{Visible and hierarchical neural network architecture for real-time phantom limb generation.}

It is known that any system can be regarded as a hierarchical structure (i.e., system $\rightarrow$ subsystem $\rightarrow$ subsubsystem, \ldots). As illustrated in Figure \ref{Fig3B-VisibleHierarchicalNN}(a), the human body system can be always divided into sub-components that are mechanically correlated. Inspired by the Bayesian network, we propose a visible and hierarchical neural network (VHNN) to accurately formulate a system. As illustrated in 
Figure \ref{Fig3B-VisibleHierarchicalNN}(b), a sample visible and hierarchical neural network, which is directly derived from the human body system, is employed to specify the musculoskeletal kinematic. The visible and hierarchical neural network can be employed in phantom limb generation, 4D kinetic behavior recognition, and individualized Tai-Chi choreography (to be discussed in the remaining sections). 
Preliminary experimental results demonstrate that VHNN is superior to a classical neural network from the point of view of training speed and stability. 

%A more detailed discussion will be make in subsection \ref{subsection:compensationMissingData}. 
\begin{wrapfigure}{L}{0.6\textwidth}
     \centering
     \includegraphics[width=0.6\textwidth]{figures/fig03B-VisibleHierarchicalNN.jpg}
 	\caption{Visible and hierarchical neural network}
 	\label{Fig3B-VisibleHierarchicalNN}
 	\vspace{-2mm}
\end{wrapfigure}


\subsection{Generating phantom legs based on arm movement using visible and hierarchical autoencoder network.}

As our preliminary contribution, a neural network is trained to generate the kinetic status of hip, knees, and feet according to the kinetic status of shoulders, elbows, and arms captured by 4D sensors \cite{online13-Dakila-Autoencoder-PhantomLeg2018}.
As illustrated in Figure \ref{Fig16CDE-autoencoder-phantomLegs}, four network architectures are investigated in this research: (a) multiple layer perceptron (MLP); (b) denoising autoencoder (a classical autoencoder architecture); (c) visible and hierarchical neural network with two subsystems (VHNN2); and (c) VHNN with four subsystems (VHNN4). 
It can be observed that VHNN splits the input tensor and then feeds the split tensor into multiple smaller, parallelized autoencoders. Thus, data for each joint can be calculated in parallel with their own respective autoencoder. The aforementioned parallelized autoencoder pipelines are simplified stacked autoencoders, allowing for optimization of specific, key tasks rather than one large task.
A video playlist of the generation of phantom legs based on VHNN may be found at 
\cite{online20-Dakila-PhantomLeg2018}.
%% \textcolor{red}{https://www.youtube.com/playlist?list=PL8VO3nxhbh0IngDo5ij0PkKxK5uFbtXE0.}
%% Cite this instead

% \begin{figure}[htp]
%  	\centering
% 	\includegraphics[height=4.5 cm]{figures/fig16C-SingleThread-Encoder-PhantomLeg.jpg}
% 	\hspace{2cm}
% 	\includegraphics[height=4.5 cm]{figures/fig16G-MLP-phantomLegs.jpg}
% 	\caption{Preliminary result about  MLP phantom legs generation: (a) architecture of MLP; (b) walking by moving arms (https://www.youtube.com/watch?v=BFW3JVI0dKM ).
% 	}
% 	\label{Fig16CD-MLP-phantomLegs}
% \end{figure} 



\begin{table}[htp]
\centering
\caption{Time-performance of phantom-legs generation using visible and hierarchical autoencoder neural network (VHNN) (Intel Core i9-7900X, 1x NVIDIA GTX1080 Ti, 64GB RAM; MLP does not employ GPU)}
	\begin{tabular}{|l|l|l|l|l|l|}
		\hline
		NN architecture	 & Training time  & Training time & convergence    & ground      & online \\ 
		                 & per step       & for 1K epochs & in epoch      & truth error  &     video   \\ \hline
		MLP					  & NA   			 & NA       &  ~250  &   9515.51  &  \cite{online14-Dakila-MLP-PhantomLeg2018}\\
		Denoising Autoencoder & $108-110\mu s$   & 9m 15s   &  ~1000 &   2107.46  & \cite{online15-Dakila-MLP-PhantomLeg2018}\\
		VPNN-Autoencoder-2	  & $30-31\mu s$	 &  2m 44s      &  ~500     &   276.68       & \cite{online16-Dakila-MLP-PhantomLeg2018}\\
		VPNN-Autoencoder-4    & $52-57 \mu s$	 & 4m 37s   &  ~800  &   366.15   & \cite{online17-Dakila-MLP-PhantomLeg2018}\\ \hline
	\end{tabular}
\label{Table5-VHNN-phantom-legs-generation}
\end{table}


As illustrated in Table \ref{Table5-VHNN-phantom-legs-generation}, the proposed VPNN 
 architecture has proven to have overall superior results compared to previous work. \textcolor{black}{Decreased training time compared to previous autoencoders architectures can be observed due to the parallelization of simpler autoencoders, increasing efficiency by easing optimization. This is done by allowing autoencoders to train on specific gestures in a whole movement. In addition, it does not exhibit data-hungry tendencies that state-of-the-art models exhibit, allowing it to be trained on small amounts of data.}
 
 \textcolor{black}{Lower ground truth error can be seen in the VPNN-AE-2 versus VPNN-AE-4. This is due to training data having no anomalies of data that real-time can exhibit. While VPNN-AE-2 with single-correlation works better when testing against ground truth data, VPNN-AE-4 with double-correlation works better in real-time as the patient may not follow the Tai-Chi movements correctly. This causes worse ground truth error as the added complexity of the architecture increases noise during output, but enables better patient-error tolerance. Because of this additional noise produced of VPNN-AE-4, improvements such as larger training datasets, more sophisticated pre- and post-processing of data, as well as improvements in NN architecture will be investigated.}
 
\begin{figure}[htp]
 	\centering
 	\includegraphics[height=6 cm]{figures/fig16CC-MLP.jpg}
	\hspace{0.25cm}
	\includegraphics[height=6 cm]{figures/fig16C-SingleThread-Encoder-PhantomLeg.jpg}
	\hspace{0.25cm}
	\includegraphics[height=6 cm]{figures/fig16D-TwoThread-Encoder-PhantomLeg.jpg}
	\hspace{0.25cm}
	\includegraphics[height=6 cm]{figures/fig16E-FourThread-Encoder-PhantomLeg.jpg}
% 	\hspace{0.5cm}
% 	\includegraphics[height=4.5 cm]{figures/fig16E-VariousEncoder-PhantomLeg.jpg}
	\caption{Generation of phantom legs from moving arms using various architecture \cite{online20-Dakila-PhantomLeg2018}: (a) MLP; (b) denoising autoencoder (a classical architecture); (c) two thread (subsystem) visible and hierarchical autoencoder neural network (VHNN-AE-2); (d) four-thread VHNN (VHNN-AE-4) (notes: LL-LA indicates phantom left-leg induced by left-arm; LL-RA indicates phantom right-leg induced by right arm) (online video: \cite{online20-Dakila-PhantomLeg2018})
	%% (d) walking by moving arms (YouTUBE: https://youtu.be/eou3YVwoxIM).
	}
	\label{Fig16CDE-autoencoder-phantomLegs}
	\vspace{-4mm}
\end{figure} 

==> backup/8.clinic.tex <==
\section{Clinic Evaluation of the Proposed Work}
